Data-Driven Evolutionary Multi-Objective Optimization Based on Multiple-Gradient Descent for Disconnected Pareto Fronts

Data-driven evolutionary multi-objective optimization (EMO) has been recognized as an effective approach for multi-objective optimization problems with expensive objective functions. The current research is mainly developed for problems with a 'regular' triangle-like Pareto-optimal front (PF), whereas the performance can significantly deteriorate when the PF consists of disconnected segments. Furthermore, the offspring reproduction in the current data-driven EMO does not fully leverage the latent information of the surrogate model. Bearing these considerations in mind, this paper proposes a data-driven EMO algorithm based on multiple-gradient descent. By leveraging the regularity information provided by the up-to-date surrogate model, it is able to progressively probe a set of well distributed candidate solutions with a convergence guarantee. In addition, its infill criterion recommends a batch of promising candidate solutions to conduct expensive objective function evaluations. Experiments on $33$ benchmark test problem instances with disconnected PFs fully demonstrate the effectiveness of our proposed method against four selected peer algorithms.

==> literature.tex <==
\section{Related Works}
\label{sec:literature}
In this section we discuss related works on the current developments of data-driven EMO.
More details can be found in some excellent survey papers~\cite{Jin05,Jin11,JinWCGM19}. 

A typical way is using a set of predefined scalarizing weight vectors to convert multiple objective functions into a scalar function. EAs are used to solve this single objective function. 
Knowles~\cite{Knowles06} turns the multi-objective problem into a single objective problem based on a random weight vector. Then EA is used to optimize this scalarizing function. 
Emmerich et al.~\cite{EmmerichGN06,EmmerichDK11} proposed a variant following ParEGO, using Hypervolume measure as an alternative of scalarizing function. EA is also used to optimize this function. 

Other works build multiple surrogates to approximate the expensive objective functions and use multi-objective EAs to do the optimization. 
Zhang et al.~\cite{ZhangLTV10} proposed a MOEA/D version of EGO, dubbed MOEA/D-EGO. The GPR to fit a surrogate model for each expensive objective function and a regular MOEA/D routine is used to search for the approximated PF. 
K-RVEA~\cite{ChughJMHS18} also fit a surrogate model for each expensive objective function, while adopting RVEA~\cite{ChengJOS16} to search. 
~\cite{HabibSCRM19} proposed HSMEA that takes advantages of the interplay of multiple surrogate models and two sets of reference vectors. 

Different from the above mentioned works, some others (e.g. Loshchilov~\cite{LoshchilovSS10} and Seah et al.~\cite{SeahOTJ12}) proposed to fit a surrogate model that predicts the Pareto dominance relation between pairs of solutions.

There are a wide variety of selection strategies have been proposed, while the strategy of individual generation has not been focused. Typical crossover operator (e.g. SBX) and mutation operator (e.g. Polynomial mutation) are commonly used in the EAs part in these works, which are designed for black-box optimization. However, the optimization on the surrogate models is not black box. Most of the surrogate models have close-form.  

==> tables/RQ1-old.tex <==
\begin{table}[htbp]
	\caption{Comparison Results of \texttt{SAMOEA-MGD} with the peer algorithms} 
	\label{tab:RQ1}
	\resizebox{1.0\textwidth}{!}{ 
\begin{tabular}{c|ccc|ccc}
\cline{2-7}
\multirow{2}{*}{}                         & \multicolumn{3}{c|}{ZDT3}                                                                                                         & \multicolumn{3}{c|}{ZDT31}                                                                                                                             \\ \cline{2-7} 
                                          & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & $n=8$                         & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & \multicolumn{1}{c|}{$n=8$}                         \\ \hline
\multicolumn{1}{|c|}{\texttt{SAMOEA-MGD}} & \multicolumn{1}{c|}{\bb{1.3199(3.34E-3)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.3271(1.52E-3)}$^\dag$} & \bb{1.3260(4.29E-3)}$^\dag$ & \multicolumn{1}{c|}{\bb{1.3813(2.64E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.3706(2.74E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.3655(7.06E-2)}$^\dag$} \\ \hline
\multicolumn{1}{|c|}{\texttt{HSMEA}}      & \multicolumn{1}{c|}{1.2914(5.99E-2)}             & \multicolumn{1}{c|}{1.2888(7.93E-2)}             & 1.1901(1.53E-1)             & \multicolumn{1}{c|}{1.3183(2.06E-1)}             & \multicolumn{1}{c|}{1.3064(6.99E-2)}             & \multicolumn{1}{c|}{1.1851(1.14E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{K-RVEA}}     & \multicolumn{1}{c|}{1.1814(1.77E-1)}             & \multicolumn{1}{c|}{1.1842(7.44E-2)}             & 1.2394(1.16E-1)             & \multicolumn{1}{c|}{1.0556(2.54E-1)}             & \multicolumn{1}{c|}{1.1107(1.72E-1)}             & \multicolumn{1}{c|}{1.1098(1.65E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{MOEA/D-EGO}} & \multicolumn{1}{c|}{1.1831(9.85E-2)}             & \multicolumn{1}{c|}{1.0566(1.58E-1)}             & 1.0050(1.14E-1)             & \multicolumn{1}{c|}{1.0983(2.84E-1)}             & \multicolumn{1}{c|}{1.0351(2.13E-1)}             & \multicolumn{1}{c|}{0.9112(1.21E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{ParEGO}}     & \multicolumn{1}{c|}{1.1549(4.84E-2)}             & \multicolumn{1}{c|}{1.0364(1.57E-1)}             & 0.7974(1.09E-1)             & \multicolumn{1}{c|}{1.0839(9.35E-2)}             & \multicolumn{1}{c|}{1.0068(8.73E-2)}             & \multicolumn{1}{c|}{0.8659(2.16E-1)}             \\ \hline
\multirow{2}{*}{}                         & \multicolumn{3}{c|}{ZDT32}                                                                                                        & \multicolumn{3}{c|}{ZDT33}                                                                                                                             \\ \cline{2-7} 
                                          & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & $n=8$                         & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & \multicolumn{1}{c|}{$n=8$}                         \\ \hline
\multicolumn{1}{|c|}{\texttt{SAMOEA-MGD}} & \multicolumn{1}{c|}{\bb{1.2818(2.18E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.2610(8.73E-2)}$^\dag$} & \bb{1.2860(2.12E-2)}$^\dag$ & \multicolumn{1}{c|}{\bb{0.9089(6.31E-4)}$^\dag$} & \multicolumn{1}{c|}{\bb{0.9075(1.04E-3)}$^\dag$} & \multicolumn{1}{c|}{\bb{0.9036(7.43E-2)}$^\dag$} \\ \hline
\multicolumn{1}{|c|}{\texttt{HSMEA}}      & \multicolumn{1}{c|}{1.2309(9.73E-2)}             & \multicolumn{1}{c|}{1.1801(9.62E-2)}             & 1.1604(9.41E-2)             & \multicolumn{1}{c|}{0.8643(5.41E-2)}             & \multicolumn{1}{c|}{0.8508(3.32E-2)}             & \multicolumn{1}{c|}{0.8130(9.20E-2)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{K-RVEA}}     & \multicolumn{1}{c|}{1.1852(7.96E-2)}             & \multicolumn{1}{c|}{1.1359(6.86E-2)}             & 1.1550(8.02E-2)             & \multicolumn{1}{c|}{0.8683(7.07E-2)}             & \multicolumn{1}{c|}{0.8845(6.85E-2)}             & \multicolumn{1}{c|}{0.8630(6.48E-2)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{MOEA/D-EGO}} & \multicolumn{1}{c|}{1.1265(4.74E-2)}             & \multicolumn{1}{c|}{1.0960(6.78E-2)}             & 1.0355(1.04E-1)             & \multicolumn{1}{c|}{0.8578(3.22E-2)}             & \multicolumn{1}{c|}{0.8148(1.83E-2)}             & \multicolumn{1}{c|}{0.7911(3.25E-2)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{ParEGO}}     & \multicolumn{1}{c|}{1.1170(1.52E-2)}             & \multicolumn{1}{c|}{1.0801(1.07E-1)}             & 1.0175(1.15E-1)             & \multicolumn{1}{c|}{0.8249(2.46E-2)}             & \multicolumn{1}{c|}{0.7487(5.64E-2)}             & \multicolumn{1}{c|}{0.7126(4.45E-2)}             \\ \hline
\multirow{2}{*}{}                         & \multicolumn{3}{c|}{WFG2}                                                                                                         & \multicolumn{3}{c|}{WFG21}                                                                                                                             \\ \cline{2-7} 
                                          & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & $n=8$                         & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & \multicolumn{1}{c|}{$n=8$}                         \\ \hline
\multicolumn{1}{|c|}{\texttt{SAMOEA-MGD}} & \multicolumn{1}{c|}{\bb{5.9298(3.99E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{5.9799(3.14E-2)}$^\dag$} & \bb{5.7457(6.63E-2)}$^\dag$ & \multicolumn{1}{c|}{\bb{6.2155(4.87E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{6.2630(2.37E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{6.0309(5.79E-2)}$^\dag$} \\ \hline
\multicolumn{1}{|c|}{\texttt{HSMEA}}      & \multicolumn{1}{c|}{5.7944(2.10E-1)}             & \multicolumn{1}{c|}{5.8221(1.11E-1)}             & 5.1535(3.36E-1)             & \multicolumn{1}{c|}{5.5538(4.16E-1)}             & \multicolumn{1}{c|}{5.0867(5.17E-1)}             & \multicolumn{1}{c|}{4.5420(3.14E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{K-RVEA}}     & \multicolumn{1}{c|}{5.7083(1.48E-1)}             & \multicolumn{1}{c|}{5.4672(1.40E-1)}             & 5.1191(3.18E-1)             & \multicolumn{1}{c|}{5.5407(3.49E-1)}             & \multicolumn{1}{c|}{5.5867(9.45E-2)}             & \multicolumn{1}{c|}{5.2068(3.06E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{MOEA/D-EGO}} & \multicolumn{1}{c|}{4.9327(3.51E-1)}             & \multicolumn{1}{c|}{4.6521(4.99E-1)}             & 4.0520(4.96E-1)             & \multicolumn{1}{c|}{4.9540(3.22E-1)}             & \multicolumn{1}{c|}{4.7417(4.15E-1)}             & \multicolumn{1}{c|}{4.0720(3.10E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{ParEGO}}     & \multicolumn{1}{c|}{4.6709(2.84E-1)}             & \multicolumn{1}{c|}{4.5911(6.76E-1)}             & 3.8378(4.09E-1)             & \multicolumn{1}{c|}{4.8377(2.97E-1)}             & \multicolumn{1}{c|}{4.6174(3.08E-1)}             & \multicolumn{1}{c|}{3.9503(4.48E-1)}             \\ \hline
\multirow{2}{*}{}                         & \multicolumn{3}{c|}{WFG22}                                                                                                        & \multicolumn{3}{c|}{WFG23}                                                                                                                             \\ \cline{2-7} 
                                          & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & $n=8$                         & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & \multicolumn{1}{c|}{$n=8$}                         \\ \hline
\multicolumn{1}{|c|}{\texttt{SAMOEA-MGD}} & \multicolumn{1}{c|}{\bb{2.8400(6.29E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{2.8638(6.03E-2)}$^\dag$} & \bb{2.6378(1.14E-1)}$^\dag$ & \multicolumn{1}{c|}{\bb{5.7030(3.45E-1)}$^\dag$} & \multicolumn{1}{c|}{\bb{5.9445(9.55E-2)}$^\dag$} & \multicolumn{1}{c|}{\bb{5.6221(9.38E-2)}$^\dag$} \\ \hline
\multicolumn{1}{|c|}{\texttt{HSMEA}}      & \multicolumn{1}{c|}{2.8154(1.42E-1)}             & \multicolumn{1}{c|}{2.6386(1.21E-1)}             & 1.3896(0.00E+0)             & \multicolumn{1}{c|}{0.0000(0.00E+0)}             & \multicolumn{1}{c|}{0.0000(0.00E+0)}             & \multicolumn{1}{c|}{0.0000(0.00E+0)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{K-RVEA}}     & \multicolumn{1}{c|}{2.5958(1.55E-1)}             & \multicolumn{1}{c|}{2.3946(6.85E-2)}             & 1.8419(1.50E-1)             & \multicolumn{1}{c|}{5.4574(2.62E-1)}             & \multicolumn{1}{c|}{5.4525(1.42E-1)}             & \multicolumn{1}{c|}{4.8954(2.38E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{MOEA/D-EGO}} & \multicolumn{1}{c|}{2.0903(1.65E-1)}             & \multicolumn{1}{c|}{1.8671(1.47E-1)}             & 1.3691(5.16E-1)             & \multicolumn{1}{c|}{4.9859(2.54E-1)}             & \multicolumn{1}{c|}{4.9615(2.60E-1)}             & \multicolumn{1}{c|}{4.2413(3.71E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{ParEGO}}     & \multicolumn{1}{c|}{2.0581(1.68E-1)}             & \multicolumn{1}{c|}{1.9506(1.78E-1)}             & 1.3248(2.54E-1)             & \multicolumn{1}{c|}{5.0298(4.56E-1)}             & \multicolumn{1}{c|}{4.7642(5.69E-1)}             & \multicolumn{1}{c|}{4.0819(2.20E-1)}             \\ \hline
\multirow{2}{*}{}                         & \multicolumn{3}{c|}{DTLZ7}                                                                                                        & \multicolumn{3}{c|}{DTLZ71}                                                                                                                            \\ \cline{2-7} 
                                          & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & $n=8$                         & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & \multicolumn{1}{c|}{$n=8$}                         \\ \hline
\multicolumn{1}{|c|}{\texttt{SAMOEA-MGD}} & \multicolumn{1}{c|}{\bb{1.3234(7.52E-3)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.3330(1.29E-3)}$^\dag$} & \bb{1.3297(2.99E-3)}$^\dag$ & \multicolumn{1}{c|}{\bb{1.3996(2.64E-3)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.4040(2.96E-3)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.4034(4.42E-3)}$^\dag$} \\ \hline
\multicolumn{1}{|c|}{\texttt{HSMEA}}      & \multicolumn{1}{c|}{1.3195(1.84E-2)}             & \multicolumn{1}{c|}{1.3138(1.73E-2)}             & 1.3123(1.09E-2)             & \multicolumn{1}{c|}{1.3959(1.02E-2)}             & \multicolumn{1}{c|}{1.3936(9.43E-3)}             & \multicolumn{1}{c|}{1.3762(1.07E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{K-RVEA}}     & \multicolumn{1}{c|}{1.2407(1.18E-2)}             & \multicolumn{1}{c|}{1.2371(2.14E-2)}             & 1.2263(2.52E-2)             & \multicolumn{1}{c|}{1.3289(1.79E-2)}             & \multicolumn{1}{c|}{1.3190(1.26E-2)}             & \multicolumn{1}{c|}{1.3146(1.50E-2)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{MOEA/D-EGO}} & \multicolumn{1}{c|}{1.2550(2.56E-2)}             & \multicolumn{1}{c|}{1.2131(1.20E-1)}             & 1.1591(1.13E-1)             & \multicolumn{1}{c|}{1.2916(7.39E-1)}             & \multicolumn{1}{c|}{1.2746(3.82E-1)}             & \multicolumn{1}{c|}{1.0508(1.41E-1)}             \\ \hline
\multicolumn{1}{|c|}{\texttt{ParEGO}}     & \multicolumn{1}{c|}{1.2076(6.05E-2)}             & \multicolumn{1}{c|}{1.1303(5.55E-2)}             & 1.0667(1.21E-1)             & \multicolumn{1}{c|}{1.2735(2.84E-2)}             & \multicolumn{1}{c|}{1.0609(1.67E-1)}             & \multicolumn{1}{c|}{0.9420(2.51E-1)}             \\ \hline
\multirow{2}{*}{}                         & \multicolumn{3}{c|}{DTLZ72}                                                                                                       &                                                  &                                                  &                                                  \\ \cline{2-4}
                                          & \multicolumn{1}{c|}{$n=3$}                         & \multicolumn{1}{c|}{$n=5$}                         & $n=8$                         &                                                  &                                                  &                                                  \\ \cline{1-4}
\multicolumn{1}{|c|}{\texttt{SAMOEA-MGD}} & \multicolumn{1}{c|}{\bb{1.4013(9.67E-3)}$^\dag$} & \multicolumn{1}{c|}{\bb{1.4075(2.62E-3)}$^\dag$} & \bb{1.4052(2.34E-3)}$^\dag$ &                                                  &                                                  &                                                  \\ \cline{1-4}
\multicolumn{1}{|c|}{\texttt{HSMEA}}      & \multicolumn{1}{c|}{1.4013(1.69E-2)}             & \multicolumn{1}{c|}{1.3926(1.00E-2)}             & 1.3875(1.20E-1)             &                                                  &                                                  &                                                  \\ \cline{1-4}
\multicolumn{1}{|c|}{\texttt{K-RVEA}}     & \multicolumn{1}{c|}{1.3292(2.58E-2)}             & \multicolumn{1}{c|}{1.3313(1.72E-2)}             & 1.3170(1.53E-2)             &                                                  &                                                  &                                                  \\ \cline{1-4}
\multicolumn{1}{|c|}{\texttt{MOEA/D-EGO}} & \multicolumn{1}{c|}{1.3006(1.44E-1)}             & \multicolumn{1}{c|}{1.1908(1.14E-1)}             & 1.0411(8.06E-2)             &                                                  &                                                  &                                                  \\ \cline{1-4}
\multicolumn{1}{|c|}{\texttt{ParEGO}}     & \multicolumn{1}{c|}{1.2863(4.18E-2)}             & \multicolumn{1}{c|}{1.2150(6.59E-2)}             & 0.9540(2.36E-1)             &                                                  &                                                  &                                                  \\ \cline{1-4}
\end{tabular}
}
\end{table}
